Offshore Wind Integration in the North Sea: The Benefits of an Offshore Grid and Floating Wind

Wind energy has become increasingly important for meeting Europe's energy needs. While onshore wind expansion faces public acceptance problems, for offshore wind the European Commission has introduced ambitious goals to increase capacity from 15GW to 300GW in 2050. Incorporating more offshore wind electricity into the power grid may offer a more widely accepted way to satisfy Europe's energy demand. In particular, the North Sea region has large potential for offshore wind generation. However, to fully exploit the wind potential in the North Sea, the grid integration of offshore wind and floating wind turbines are vital, especially when onshore wind capacity and onshore grid expansion are constrained. For the grid integration, a meshed offshore grid can offer a viable alternative to the standard direct connection of offshore wind parks to the nearest point on land combined with point-to-point HVDC connections. In this paper, we investigate the benefits of having a meshed offshore grid in the North Sea and considering floating wind besides fixed-bottom wind installations. In our analysis, we look at eight different scenarios, where onshore wind potentials and onshore line expansion are limited, to explore the effects of low public acceptance. Our results demonstrate that the presence of an offshore grid can reduce total system costs by up to 2.6 bn Euro/a. In the scenarios with an offshore meshed grid, ~8% more offshore wind capacities are built compared to the scenarios without a meshed grid. Furthermore, the analysis shows that if onshore wind potentials are restricted, floating wind turbines play a key role and compensate for lacking onshore wind capacities.

==> structure.tex <==

\usepackage[
nochapters, %
beramono, %
eulermath,%
pdfspacing, %
dottedtoc %
]{classicthesis} %

\usepackage{arsclassica} %

\usepackage[T1]{fontenc} %

\usepackage[utf8]{inputenc} %

\usepackage{graphicx} %
\graphicspath{{Figures/}} %

\usepackage{enumitem} %

\usepackage{lipsum} %

\usepackage{subfig} %

\usepackage{amsmath,amssymb,amsthm} %

\usepackage{varioref} %


\usepackage[left=2cm,right=2cm,top=1.5cm,bottom=1cm]{geometry}

\usepackage[printonlyused]{acronym}

\usepackage{graphicx}

\usepackage{cleveref}

\theoremstyle{definition} %
\newtheorem{definition}{Definition}

\theoremstyle{plain} %
\newtheorem{theorem}{Theorem}

\theoremstyle{remark} %


\hypersetup{
colorlinks=true, breaklinks=true, bookmarks=true,bookmarksnumbered,
urlcolor=webbrown, linkcolor=RoyalBlue, citecolor=webgreen, %
pdftitle={}, %
pdfauthor={\textcopyright}, %
pdfsubject={}, %
pdfkeywords={}, %
pdfcreator={pdfLaTeX}, %
pdfproducer={LaTeX with hyperref and ClassicThesis} %
}


\usepackage[%
 backend=biber,bibencoding=utf8, %
  language=auto,%
  style=numeric-comp,%
  sorting=none, %
  maxbibnames=10, %
  natbib=true %
]{biblatex}



\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}






